Search for long-lived particles in final states with displaced dimuon vertices in $pp$ collisions at $\sqrt{s}=$ 13 TeV with the ATLAS detector

A search is performed for a long-lived particle decaying into a final state that includes a pair of muons of opposite-sign electric charge, using proton-proton collision data collected at $\sqrt{s}=$ 13 TeV by the ATLAS detector at the Large Hadron Collider corresponding to an integrated luminosity of 32.9 fb$^{-1}$. No significant excess over the Standard Model expectation is observed. Limits at 95% confidence level on the lifetime of the long-lived particle are presented in models of new phenomena including gauge-mediated supersymmetry or decay of the Higgs boson, $H$, to a pair of dark photons, $Z_D$. Lifetimes in the range c$\tau$ = 1-2400 cm are excluded, depending on the parameters of the model. In the supersymmetric model, the lightest neutralino is the next-to-lightest supersymmetric particle, with a relatively long lifetime due to its weak coupling to the gravitino, the lightest supersymmetric particle. The lifetime limits are determined for very light gravitino mass and various assumptions for the neutralino mass in the range 300 GeV to 1000 GeV. In the dark photon model, the lifetime limits are interpreted as exclusion contours in the plane of the coupling between the $Z_D$ and the Standard Model $Z$ boson versus the $Z_D$ mass (in the range 20-60 GeV), for various assumptions for the $H\rightarrow Z_D Z_D$ branching fraction.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 24-Oct-2018

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DRF/IRFU, France; SRNSFG, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, CANARIE, CRC and Compute Canada, Canada; COST, ERC, ERDF, Horizon 2020, and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d' Avenir Labex and Idex, ANR, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF, Greece; BSF-NSF and GIF, Israel; CERCA Programme Generalitat de Catalunya, Spain; The Royal Society and Leverhulme Trust, United Kingdom. 

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------


